A review on reinforcement learning methods for mobility on demand systems

Mobility on Demand (MoD) refers to mobility systems that operate on the basis of immediate travel demand. Typically, such a system consists of a fleet of vehicles that can be booked by customers when needed. The operation of these services consists of two main tasks: deciding how vehicles are assigned to requests (vehicle assignment); and deciding where vehicles move (including charging stations) when they are not serving a request (rebalancing). A field of research is emerging around the design of operation strategies for MoD services, and an increasingly popular trend is the use of learning based (most often Reinforcement Learning) approaches. We review, in this work, the literature on algorithms for operation strategies of MoD systems that use approaches based on Reinforcement Learning with a focus on the types of algorithms being used. The novelty of our review stands in three aspects: First, the algorithmic details are discussed and the approaches classified in a unified framework for sequential decision-making. Second, the use cases on which approaches are tested and their features are taken into account. Finally, validation methods that can be found across the literature are discussed. The review aims at advancing the state of the art by identifying similarities and differences between approaches and highlighting current research directions.

==> 5_Discussion.tex <==
\section{Discussion and Conclusion}

Similarly to our analysis, we articulate the discussion around the three dimensions of algorithmic basis; the use case aspects; and the methodology. 

On the algorithmic side, even though value function approximation is used in most of the literature detailed in this work, one type of value function approximation is mostly used for the operation of MoD system, that is neural networks. However, as noted in section \ref{background}, in the literature of Reinforcement Learning various approximation techniques are used and deserve to be explored in the context of MoD operation. Also, the research in this area would benefit from more exploration of PFA techniques.


Regarding the use cases on which the algorithms are evaluated, agent-based simulators that allow a high level of detail are theoretically used. However, it is surprising that congestion and presence of public transports are not always taken into account. Also, we find that there is considerable potential in presenting more detailed analysis regarding different profiles of users. Moreover, the studied use cases mostly reflect urban settings, the potential of MoD in rural setting has been demonstrated in the literature and its operation on such use cases using RL techniques is worth investigating. A recurrent aspect in the literature is the consideration of a uniform and often unrealistic population with similar trips and characteristics. An emergent practice is the use of synthetic populations that are generated from various socio-economic data to reflect the real population. In general, we estimate that future works should consider a wider variety of features.

Regarding other methodological aspects, sensitivity analyses on the parameters that are specific to each approach are not always presented, while they could give useful insights on the performance of the approach and its scalability. E.g, the number of considered zones, the learning rate, the discount factor... The same applies to use-case related parameters: fleet size, vehicle capacity... 
Also, while some approaches use abstract representation that are argued to be transferrable, no example was shown with where the learning performed on one use case was transferred and carried on with another use case. 
Another major point that is raised is the comparisons performed in the different papers. The proposed approaches are rarely tested against other RL approaches proposed elsewhere in the literature, and the benchmarks are very often performed in comparison with classical approaches defined within the studies. This can be explained by a lack of comprehensive benchmark in the literature in which algorithms (taking into account various features) can be implemented and compared. The only occurrence of common benchmarking of RL based algorithms for MoD operation that we have encountered in our review was the KDD RL cup competition, for which \cite{tang_value_2021} has been submitted. This is strongly related to the notion of reproducibility of the results presented in the papers, both in terms of details regarding the approach and the methodology and in terms of openness of data that are used to build the use cases on which they are tested. What is surprising here is that none of the mentioned papers is completely and easily reproducible. Ideally, a link to the necessary data and to a repository containing the source code should be provided.

Consequently, we recommend the following pathways of research around the use of RL based method (and other methods) for MoD operation: a comprehensive test case including an extensive set of features and relying on open-data should be proposed. The test case should be based on a modular open-source simulation tool that can be extended with various algorithms that can then be tested against each other under the same case. The benchmark can start with standard out of the shelf approaches and then be expanded with more complex and novel methods. 


% On the first one, we consider that other value function approximators can be explored for the task of MoD operation. As presented in the background section regarding RL,  Also, some approaches use a representation that is dependent on the network and thus hardly transferable while others use more general representations (taking into account only the local environment). The research around the operation of MoD services mainly supposes that they are implemented using AVs that are electric, however no algorithm that uses learning explicitly considers the recharging aspect of these vehicles. Similarly, the interaction between MoD and public transport is not always explicitly taken into account. We estimate that the a proper integration of MoD with public transports represents an important feature that deserves more exploration. 

%Regarding the use cases, not all papers systematically discuss the impact of both use case parameters and approach specific parameters on their performance. Most papers compare the approach they present to other simple algorithms that are developed in the scope of the project for the sake of illustration. This is related to the fact that some approaches are also more reproducible than others.  The use of built-in simulators and the varying level of details in the presentation of different approaches makes reproducibility and comparison to other approaches hard to achieve. These aspects can be improved by introducing more openness to the approaches: openness of data (publicly available traffic and travel demand data), openness of tools (simulation framework and optimization tools), and openness of algorithms by providing enough details to allow researches to fully reproduce the results. 

% The use cases are strongly related to the features taken into account by the algorithms, public transport and private vehicles are not always taken into account in the simulated scenarios. Even if the algorithms do not explicitly consider these aspects, we consider that it is important to include them in simulation of MoD services to study the impact on modal shares. This would allow a more realistic and comprehensive assessment of the impact a studied system would have.  Finally, although some algorithms use representations that can be transferred accross different road networks, no research illustrates the use on a scenario of a strategy learned on another scenario.

% Assembling the three dimensions together, we are able to propose a concrete path for development in this field.  More precisely, we consider that a reachable and a reasonable goal (given the current state of the literature and the openly available tools and methodologies that can be extended) to set is the design of an MoD operation/rebalancing/dispatch algorithm that features: management of electric batteries and recharging, interaction with public transport, ability to generalize on other networks/scenarios.  The performance of such an algorithm should be assessed in a realistic scenario and in an intermodal setting. To evaluate transferability to other settings, the learning on a second scenario should be studied by comparing the use of the policy learned in a first scenario against performing the learning without initial knowledge. Also, we suggest some high level guidelines for future works to make the research in this area more robust: sensitivity analysis of both scenario settings and approach parameters; use open simulation tools and open scenarios; allow reproducibility of new approaches (in the best case the implementation's code would be publicly available but we consider that at least enough details should be presented to allow other research to re-implement the algorithms)



%This area of research is witnessing an expanding interest from the research community. We consequently present a brief overview of the emerging research composed of still-under-review articles and published abstracts. Another development performed upon the work described in \citep{al-abbasi_deeppool_2019} is proposed in \cite{qian2021drop} to tackle the issue of exploration under environments with sparse rewards and unbalanced demand and supply levels. This approach is evaluated using historical New York trips data. In \citep{jiao2021real}, a deep reinforcement learning algorithm with a SARSA architecture is used for the rebalancing task with an emphasis on large fleets and real world settings. In this research specifically and in addition to evaluation in simulation, the proposed algorithms were tested by real MoD fleets of varying sizes in different cities. \citet{lei2020efficient} uses recurrent neural networks for the rebalancing task and evaluates this approach in simulation using New York trips data.

In this review, we have presented the current state of the research related to the use of learning based approaches for the operation of on-demand mobility in agent-based simulations.
Rather than a systematic review, ours highlights the various algorithmic techniques that are used and locate them in respects to a general framework. 
We also consider the uses cases in which different approaches are tested and the practices that are followed to evaluate them. 
Our research identifies gaps on these three dimensions and we outline pathways for future developments and propose guidelines to steer the research in this order to become more robust and reproducible. 


==> 6_Conclusion.tex <==
\section{Conclusion}

% We conclude and lay out some perspectives and announce our future work explicitly considering ridesharing, electric vehicles and public transport at the same time.




==> table_1.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cc|cc|ccc|c|}
\hline
reference                              & \multicolumn{2}{c|}{other modes}                                                                 & \multicolumn{2}{c|}{Sensitivity Analysis}                                                                                                                                        & \multicolumn{3}{c|}{Model Evaluation}                                                                                                                                                                                                                            & reproducibility \\ \hline
                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}along \\ private \\ cars\end{tabular}} & along PT & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}scenario \\ setup \\ parameters\end{tabular}}          & \begin{tabular}[c]{@{}c@{}}approach\\ specific\\ parameters\end{tabular} & \multicolumn{1}{c|}{simulation}                                                                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}studied \\ area\end{tabular}}                         & \begin{tabular}[c]{@{}c@{}}area \\ type\end{tabular} &                 \\ 
                                       \hline
\cite{fluri_learning_2019}             & \multicolumn{1}{c|}{No}                                                                & No        & \multicolumn{1}{c|}{No}                                                                               & Yes                                                                      & \multicolumn{1}{c|}{MATSim (AMoDeus)}                                                              & \multicolumn{1}{c|}{San Francisco}                                                                   & Urban                                                & 3
\\ \hline
\citet{wen_rebalancing_2017}           & \multicolumn{1}{c|}{No}                                                               & No       & \multicolumn{1}{c|}{Yes}                                                                              & No                                                                       & \multicolumn{1}{c|}{A grid environment}                                                            & \multicolumn{1}{c|}{Orpington, London}                                                               & Urban                                                & 2 
\\ \hline
\cite{yoshida_distributed_2021}        & \multicolumn{1}{c|}{No}                                                               & No       & \multicolumn{1}{c|}{Yes}                                                                              & Yes                                                                      & \multicolumn{1}{c|}{A grid environment}                                                            & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 0,5        
\\ \hline
\cite{kim_optimizing_2021}             & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{No}                                                                               & No                                                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the \\ project\end{tabular}} & \multicolumn{1}{c|}{Seoul}                                                                           & Urban                                                & 1   \\ \hline
\cite{gammelli2021graph}               &            \multicolumn{1}{c|}{No}                & No     & \multicolumn{1}{c|}{Multiple scenarios}    & No    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}     & \multicolumn{1}{c|}{New York and Chengdu} & Urban & 3
                                \\ \hline

    \cite{guoyang_qin_optimal_2020}        & \multicolumn{1}{c|}{No}                                                               & No       & \multicolumn{1}{c|}{No}                                                                               & Yes                                                                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}  & \multicolumn{1}{c|}{Shanghai}                                                                        & Urban                                                & 0,5       \\ \hline
\cite{enders2022hybrid}     & \multicolumn{1}{c|}{No}   & No    & \multicolumn{1}{c|}{Fleet size}   & Yes   & \multicolumn{1}{c|}{A grid environment}    &   \multicolumn{1}{c|}{New York}    &   Urban   & 1 

\\ \hline
\cite{gueriau_shared_2020}             & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{Fleet Size}                                                                       & No                                                                       & \multicolumn{1}{c|}{Sumo}                                                                          & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 2               \\ \hline
\cite{al-abbasi_deeppool_2019}         & \multicolumn{1}{c|}{No}                                                               & No       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Fleet Size\\ (Number of\\ used vehicles)\end{tabular}} & Yes                                                                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}  & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 0,5                          \\ \hline
\cite{haliem_adapool_2022}             & \multicolumn{1}{c|}{No}                                                               & No       & \multicolumn{1}{c|}{No}                                                                               & Yes                                                                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}  & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 0,5             \\ \hline 
%\cite{skordilis_modular_2021}          & \multicolumn{1}{c|}{}                                                                 &          & \multicolumn{1}{c|}{}                                                                                 &                                                                          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Buil-in agent based\\ simulator\end{tabular}}       & \multicolumn{1}{c|}{}                                                                                & Urban                                                & 0,5             \\ \hline
\citet{mao_dispatch_2020}              & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{No}                                                                               & No                                                                       & \multicolumn{1}{c|}{A grid environment}                                                            & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 2               \\ \hline
\cite{tang_value_2021}                 & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{No}                                                                               & No                                                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}DiDi simulation\\ platform\end{tabular}}            & \multicolumn{1}{c|}{?}                                                                               & Urban                                                & 2                  \\ \hline
\cite{liang_mobility-aware_2021}       & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{Yes}                                                                              & Yes                                                                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}  & \multicolumn{1}{c|}{Haikou city, China}                                                              & Urban                                                & 1               \\ \hline
\cite{castagna_demand-responsive_2021} & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{No}                                                                               & No                                                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}  & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 2               \\ \hline
%\citet{feng_coordinating_2022}         & \multicolumn{1}{c|}{Yes}                                                              & Yes      & \multicolumn{1}{c|}{No}                                                                               & No                                                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A simulator\\ built in the\\ project\end{tabular}}  & \multicolumn{1}{c|}{Manhattan}                                                                       & Urban                                                & 2               \\ \hline
%\citet{eshkevari_reinforcement_2022}   & \multicolumn{1}{c|}{Yes}                                                              & No       & \multicolumn{1}{c|}{No}                                                                               & No                                                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}DiDi simulation\\ platform\end{tabular}}            & \multicolumn{1}{c|}{?}                                                                               & Urban                                                & 2               \\ \hline
\end{tabular}
}
\caption{Analysis of the reviewed algorithms} 
\label{Table_1}
\end{table}


==> table_2.tex <==

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|}
\hline
reference                              & operation aspects        & ride sharing & recharging & policy type \\ \hline
\cite{fluri_learning_2019}             & rebalancing              & no           & no         & CFA         \\ \hline \citet{wen_rebalancing_2017}           & rebalancing              & yes          & no         & VFA         \\ \hline \cite{yoshida_distributed_2021}        & rebalancing              & yes          & no         & VFA         \\ \hline
\cite{kim_optimizing_2021}             & rebalancing              & no           & no         & VFA         \\ \hline
\cite{gammelli2021graph}               &    rebalancing             & no            & no         & CFA \\ \hline 
\cite{guoyang_qin_optimal_2020}        & dispatch                 & no           & no         & CFA         \\ \hline
\cite{enders2022hybrid} & dispatch & yes & no & CFA \\ \hline
\cite{gueriau_shared_2020} & rebalancing and dispatch & yes  & no & VFA         \\ \hline
\cite{al-abbasi_deeppool_2019}         & rebalancing and dispatch & yes          & no         & VFA         \\ \hline
%\cite{skordilis_modular_2021}          & rebalancing              &              &            & VFA         \\ \hline
\cite{haliem_adapool_2022} & rebalancing and dispatch & yes & no & VFA \\ \hline
\citet{mao_dispatch_2020} & rebalancing and dispatch & yes & no & PFA \\ \hline
\cite{tang_value_2021} & rebalancing and dispatch & no & no  & CFA \\ \hline
\cite{liang_mobility-aware_2021} & rebalancing and dispatch & no & yes & CFA\\ \hline
\cite{castagna_demand-responsive_2021} & rebalancing and dispatch & yes          & no         & PFA         \\ \hline
\end{tabular}
\caption{Classification of reviewed algorithms regarding the MoD operation tasks that are performed and their categorization in the framework presented in \citep{powell_unified_2019}} 
\label{Table_2}
\end{table}


==> table_3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|cc|cc|ccc|}
\hline
reference                              & \begin{tabular}[c]{@{}c@{}}operation \\ aspects\end{tabular}        & ridesharing & recharging & \begin{tabular}[c]{@{}c@{}}policy \\ type\end{tabular} & \multicolumn{2}{c|}{other modes}                                                                                                            & \multicolumn{2}{c|}{sensitivity analyses}                                                                                                                                 & \multicolumn{3}{c|}{model evaluation}                                                                                                                                                               \\ \hline
                                       &                                                                     &             &            &                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}along \\ private \\ cars\end{tabular}} & \begin{tabular}[c]{@{}c@{}}along \\ PT\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}scenario \\ setup \\ parameters\end{tabular}} & \begin{tabular}[c]{@{}c@{}}approach\\  specific \\ parameters\end{tabular} & \multicolumn{1}{c|}{simulation}                                                             & \multicolumn{1}{c|}{studied area}                                                         & area type \\ \hline
\cite{fluri_learning_2019}             & rebalancing                                                         & no          & no         & CFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{no}                                                                      & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}MATSim \\ (AMoDeus)\end{tabular}}            & \multicolumn{1}{c|}{San Francisco}                                                        & urban     \\ \hline
\citet{wen_rebalancing_2017}           & rebalancing                                                         & yes         & no         & VFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{yes}                                                                     & no                                                                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}grid \\ environment\end{tabular}}            & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Orpington\\ London\end{tabular}}           & urban     \\ \hline
\cite{yoshida_distributed_2021}        & rebalancing                                                         & yes         & no         & VFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{yes}                                                                     & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}grid \\ environment\end{tabular}}            & \multicolumn{1}{c|}{Manhattan}                                                            & urban     \\ \hline
\cite{kim_optimizing_2021}             & rebalancing                                                         & no          & no         & VFA                                                    & \multicolumn{1}{c|}{yes}                                                              & no                                                  & \multicolumn{1}{c|}{no}                                                                      & no                                                                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ simulator\end{tabular}}          & \multicolumn{1}{c|}{Seoul}                                                                & urban     \\ \hline
\cite{gammelli2021graph}               & rebalancing                                                         & no          & no         & CFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}multiple\\ scenarios\end{tabular}}            & no                                                                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ simulator\end{tabular}}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}New York \\ and Chengdu\end{tabular}}      & urban     \\ \hline
\cite{guoyang_qin_optimal_2020}        & dispatch                                                            & no          & no         & CFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{no}                                                                      & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ \\ simulator\end{tabular}}       & \multicolumn{1}{c|}{Shanghai}                                                             & urban     \\ \hline
\cite{enders2022hybrid}                & dispatch                                                            & yes         & no         & CFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{fleet size}                                                              & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}grid \\ environment\end{tabular}}            & \multicolumn{1}{c|}{New York}                                                             & urban     \\ \hline
\cite{gueriau_shared_2020}             & \begin{tabular}[c]{@{}c@{}}rebalancing\\ and dispatch\end{tabular}  & yes         & no         & VFA                                                    & \multicolumn{1}{c|}{yes}                                                              & no                                                  & \multicolumn{1}{c|}{fleet size}                                                              & no                                                                         & \multicolumn{1}{c|}{Sumo}                                                                   & \multicolumn{1}{c|}{Manhattan}                                                            & urban     \\ \hline
\cite{al-abbasi_deeppool_2019}         & \begin{tabular}[c]{@{}c@{}}rebalancing \\ and dispatch\end{tabular} & yes         & no         & VFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}fleet size \\ (used vehicles)\end{tabular}}   & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ simulator\end{tabular}}          & \multicolumn{1}{c|}{Manhattan}                                                            & urban     \\ \hline
\cite{haliem_adapool_2022}             & \begin{tabular}[c]{@{}c@{}}rebalancing \\ and dispatch\end{tabular} & yes         & no         & VFA                                                    & \multicolumn{1}{c|}{no}                                                               & no                                                  & \multicolumn{1}{c|}{no}                                                                      & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ simulator\end{tabular}}          & \multicolumn{1}{c|}{Manhattan}                                                            & urban     \\ \hline
\citet{mao_dispatch_2020}              & \begin{tabular}[c]{@{}c@{}}rebalancing \\ and dispatch\end{tabular} & yes         & no         & PFA                                                    & \multicolumn{1}{c|}{yes}                                                              & no                                                  & \multicolumn{1}{c|}{no}                                                                      & no                                                                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}grid \\ environment\end{tabular}}            & \multicolumn{1}{c|}{Manhattan}                                                            & urban     \\ \hline
\cite{tang_value_2021}                 & \begin{tabular}[c]{@{}c@{}}rebalancing \\ and dispatch\end{tabular} & no          & no         & CFA                                                    & \multicolumn{1}{c|}{yes}                                                              & no                                                  & \multicolumn{1}{c|}{multiple cities}                                                         & no                                                                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}DiDi \\ simulation \\ platform\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}undefined cities \\ in China\end{tabular}} & urban     \\ \hline
\cite{liang_mobility-aware_2021}       & \begin{tabular}[c]{@{}c@{}}rebalancing \\ and dispatch\end{tabular} & no          & yes        & CFA                                                    & \multicolumn{1}{c|}{yes}                                                              & no                                                  & \multicolumn{1}{c|}{yes}                                                                     & yes                                                                        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ simulator\end{tabular}}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Haikou city\\ China\end{tabular}}          & urban     \\ \hline
\cite{castagna_demand-responsive_2021} & \begin{tabular}[c]{@{}c@{}}rebalancing \\ and dispatch\end{tabular} & yes         & no         & PFA                                                    & \multicolumn{1}{c|}{yes}                                                              & no                                                  & \multicolumn{1}{c|}{no}                                                                      & no                                                                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}built-in \\ simulator\end{tabular}}          & \multicolumn{1}{c|}{Manhattan}                                                            & urban     \\ \hline
\end{tabular}
\caption{Overview of the detailed papers and the features of presented approaches}
\label{table}
\end{table}
\end{landscape}
